FOLIO: Natural Language Reasoning with First-Order Logic

Large language models (LLMs) have achieved remarkable performance on a variety of natural language understanding tasks. However, existing benchmarks are inadequate in measuring the complex logical reasoning capabilities of a model. We present FOLIO, a human-annotated, logically complex and diverse dataset for reasoning in natural language (NL), equipped with first-order logic (FOL) annotations. FOLIO consists of 1,430 examples (unique conclusions), each paired with one of 487 sets of premises used to deductively reason for the validity of each conclusion. The logical correctness of the premises and conclusions is ensured by their FOL annotations, which are automatically verified by an FOL inference engine. In addition to the main NL reasoning task, NL-FOL pairs in FOLIO constitute a new NL-FOL translation dataset. Our experiments on FOLIO systematically evaluate the FOL reasoning ability of supervised fine-tuning on medium-sized language models. For both NL reasoning and NL-FOL translation, we benchmark multiple state-of-the-art language models. Our results show that a subset of FOLIO presents a challenge for one of the most capable {Large Language Model (LLM)} publicly available, GPT-4.

==> main/tables/NL-FOL_prompt.tex <==
\begin{table*}
\footnotesize

\begin{tabular}{|p{\linewidth}|}
\hline\\
Translate the following sentences into first-order logic:
\\Premises:
\\0. Quincy McDuffie is an American professional wide receiver in Canadian Football.
\\1. People who can catch balls are good wide receivers. 
\\2. Quincy McDuffie can catch many footballs easily.
\\3. Good wide receivers play professionally.
\\4. Good wide receivers can catch with both their left and right hand.
\\5. [BG] All footballs are balls.
\\Conclusions: 
\\0. Quincy McDuffie is a good wide receiver.
\\1. Quincy McDuffie can catch every ball.
\\2. Professional wide receivers are good at catching balls.
\\Translation results are as follows: 
\\Premises:
\\0. American(quincymcduffie) $\land$ Professional(quincymcduffie) $\land$ WideReciever(quincymcduffie) $\land$ In(quincymcduffie, canadianfootball)
\\1. $\forall$x $\exists$y (CanCatch(x, y) $\land$ Ball(y) $\rightarrow$ Good(x, widereciever))
\\2. $\exists$x (Football(x) $\land$ CanCatch(quincymcduffie, x))
\\3. $\forall$x (Good(x, widereciever) $\rightarrow$ Professional(x))
\\4. $\forall$x (Good(x, widereciever) $\rightarrow$ CanCatchWith(x, lefthand) $\land$ CanCatchWith(x, righthand))
\\5. $\forall$x (Football(x) $\rightarrow$ Ball(x))
\\Conclusions: 
\\0. Good(quincymcduffie, widereciever)
\\1. $\forall$x (Ball(x) $\rightarrow$ CanCatch(quincymcduffie, x))
\\2. $\forall$x (Professional(x) $\land$ WideReciever(x) $\rightarrow$ Good(x, catchingballs))
\\\#\#\# 
\\Translate the following sentences into first-order logic:
\\Premises: 
\\0. All volunteers receive intangible benefits for their work.
\\1. Volunteers work regularly or on an as-needed basis.
\\2. Some volunteers are trained.
\\3. Volunteers work in groups or individually.
\\4. Environmental volunteers contribute toward environmental management or conservation.
\\5. Participating in natural disaster response is an example of volunteers working in groups on an as-needed basis.
\\Conclusions:
\\0. Volunteers who participate in natural disaster response receive intangible benefits for their work.
\\1. Environmental volunteers work in groups.
\\2. To be a volunteer, you must be trained.
\\Translation results are as follows: 
\\Premises: 
\\0. $\forall$x (Volunteer(x) $\rightarrow$ GetIntangibleBenefits(x))
\\1. $\forall$x (Volunteer(x) $\rightarrow$ WorkRegularly(x) $\lor$ WorkAsNeeded(x))
\\2. $\exists$x (Volunteer(x) $\rightarrow$ Trained(x))
\\3. $\forall$x (Volunteer(x) $\rightarrow$ (WorkInGroup(x) $\lor$ WorkIndividually(x)))
\\4. $\forall$x (Volunteer(x) $\land$ Environmental(x) $\rightarrow$ (ContributeTo(x, environmentalmanagement) $\lor$ ContributeTo(x, environmentalconservation)))
\\5. $\exists$x (Volunteer(x) $\land$ ContributeTo(x, naturaldisasterresponse) $\rightarrow$ WorkInGroup(x) $\land$ WorkAsNeeded(x))
\\Conclusions:
\\0. $\forall$x (Volunteer(x) $\land$ ContributeTo(x, naturaldisasterresponse) $\rightarrow$ GetIntangibleBenefits(x))
\\1. $\forall$x (Volunteer(x) $\land$ Environmental(x) $\rightarrow$ WorkRegularly(x))
\\2. $\forall$x (Volunteer(x) $\rightarrow$ Trained(x))
\\\#\#\#
\\ \textcolor{blue}{(... abbreviate ... )}
\\\#\#\#
\\Translate the following sentences into first-order logic:
\\Premises:
\\0. If people perform in school talent shows often, then they attend and are very engaged with school events.
\\1. People either perform in school talent shows often or are inactive and disinterested members of their community.
\\2. If people chaperone high school dances, then they are not students who attend the school.
\\3. All people who are inactive and disinterested members of their community chaperone high school dances.
\\4. All young children and teenagers who wish to further their academic careers and educational opportunities are students who attend the school.
\\5. Bonnie either both attends and is very engaged with school events and is a student who attends the school, or she neither attends and is very engaged with school events nor is a student who attends the school. 
\\Conclusions:
\\0. Bonnie performs in school talent shows often.
\\Translation results are as follows: 
\\
\hline
\end{tabular}
\caption{8-shot NL-FOL translation prompt.}\label{translation_prompt}
\label{tab:nl-folprompt}
\end{table*}

